On Distributed Gravitational N-Body Simulations

The N-body problem is a classic problem involving a system of N discrete bodies mutually interacting in a dynamical system. At any moment in time there are N*(N - 1)/2 such interactions occurring. This scaling as N^2 leads to computational difficulties where simulations range from tens of thousands of bodies to many millions. Approximation algorithms, such as the famous Barnes-Hut algorithm, simplify the number of interactions to scale as N(log N). Even still, this improvement in complexity is insufficient to achieve the desired performance for very large simulations on computing clusters with many nodes and many cores. In this work we explore a variety of algorithmic techniques for distributed and parallel variations on the Barnes-Hut algorithm to improve parallelism and reduce inter-process communication requirements. Explicit algorithms and details are provided for reproducibility. Our MPI implementation of distributed gravitational N-body simulation, freely available on GitHub, is evaluated on a cluster of 10 nodes, each with two 6-core CPUs, to test the effectiveness and scalability of the aforementioned techniques.

==> future.tex <==


\section{Future}

Assembly for force calc code. (e.g. ``Acceleration of the tree method with SIMD instruction set'')

==> implementation.tex <==

\section{Implementation}
\label{sec:impl}



\subsection{Data Representation}
\label{sec:dataimpl}


\subsection{Spatial Decomposition and Morton Ordering}
\label{sec:mortonimpl}


\subsection{Octrees and Hashed Octrees}
\label{sec:octreeimpl}


\subsection{Parallel Sort}
\label{sec:sortimpl}




The implementation of our treecode is written from scratch in 
the C/C++ language, making use of no external libraries.
Nearly everything is written in C, except for the 
the use of C++11 threads. Our implementation 
closely follows all of the preceding discussion, 
including the Barnes-Hut method 
described in Section~\ref{sec:bgoctree} and Algorithm~\ref{alg:BHloop}, 
the leapfrog integrator of Section~\ref{sec:leapfrog}, 
and the parallel aspects described in Section~\ref{sec:paralleltrees}.
We take this section to describe implementation-level details
which differ slightly in practice from their conceptual description
or from their original description in \cite{singh1993parallel} and \cite{DBLP:journals/jpdc/SinghHTGH95}.
In particular, we detail here our data structures, 
the use of Morton ordering to compute costzones,
our particular tree merging technique, 
and lastly, our thread implementation using the C++11 built-in \textit{thread support library}. 
Finally, we conclude with an overview of our OpenGL visualization tool.

Our main data structure is a set of parallel arrays (i.e. structure of arrays)
maintaining the masses, positions, velocities, and accelerations of the particles. 
For a particle of index $i$, its values are represented
in positions $3i$, $3i + 1$, and $3i + 2$ for the x, y, and z components, 
respectively, for each of the latter three arrays,
while mass is a simple array of scalar values.
This data layout allows our code to make use of spatial data locality 
throughout the simulation. In particular, it also
allows the use of each type of value independently 
for even better locality (cf. an array of structures).
For example, when building the tree only positions are needed, 
or when computing forces velocity is not needed.
Using this structure for the integration time-step is simple and follows 
exactly from the equations.

The only other data structure for our simulation is the tree itself.
In our case it is an octree in three dimensions. 
Our octree is a simple recursive data structure with 
each cell storing several values: 
\begin{inparaenum}[(i)]
\item its centre in physical space, 
\item its side length,
\item its centre of mass,
\item the total mass of its children,
\item the total number of particles contained in its children,
\item the quadrupole coefficients (See Equation~(\ref{eqn:truncmultipole})), and
\item a list of its 8 children if it is an internal cell.
\end{inparaenum}

To construct the octree in parallel we first determine the costzones. 
This begins with an estimate of work for each particle.
We augment our structure of arrays with one more array holding the work estimate of each particle. This array is automatically
updated during the force calculation of the previous step to count
the number of interactions
and serve as the estimate of work for the current step.\footnote{In fact, it counts not only the number of interactions but an integer value representing a work estimate. Since particle-cell interactions use quadrupole moments that particle-particle interactions do not, a particle-cell interaction is counted twice to make up for this work difference.}

Next, we must obtain a linear ordering of the particles. 
Directly using their indices as an order will not account for physical locality 
as the simulation evolves. We thus employ the Morton ordering.
In code this is referred to a \textit{spatial key}.
The Morton ordering is a bit-wise interleaving of multi-dimensional 
integer coordinates to yield a single (one-dimensional) integer which acts as key
to give the Morton ordering for the coordinates 
creating the key.
On a 64-bit machine, it is useful for this one-dimensional value
to be a single machine word. Thus each key is 64 bits and, in three dimensions,
each coordinate is a 21-bit number.
We begin by determining the bounding box of all points in the system.
Let $R$ be the smallest value such that 
all points in the system are contained in the cube with extents $[-R,R]$.
We then map each particle's floating-point coordinates from the range $[-R,R]$ to $[0, 2R]$
to $[0, 2^{21})$ and finally to an integer by taking its ceiling.
Given these three integers, it is now simple to produce the spatial key 
using Morton order bit-interleave (see \cite{warren1993parallel} for details)
or any other space-filling curve.
Each array in our structure of arrays is then sorted based on the ordering
induced by the spatial keys.

Finally, the costzones for this time-step are determined.
One simply iterates through the now sorted 
array of work estimates, aggregating contiguous partitions 
so that each partition holds $\nicefrac{1}{p}$ of the total work, given $p$ processors.
%%
Not only does this sorting yield an ordering of the particles in physical space,
but, since the structure of arrays is sorted by the spatial keys, 
spatial data locality is obtained within each costzone.
As we know, improved data locality yields improved performance.
With the costzones computed, we can now build each processor's
local octree in parallel.

Building each local tree simply follows the first step of Algorithm~\ref{alg:BHloop}.
Then, a global tree must be computed by merging each local tree.
In contrast with the original work in \cite{singh1993parallel}, 
we avoid any use of mutual exclusion to a global data structure through 
a restructuring of the merge.
Whereas all local trees were merged into a single global one, 
we merge trees pair-wise, in parallel, until only one remains, naming that 
the global one. 
The local tree construction and merge thus follows the celebrated map-reduce
parallel pattern \cite[Ch. 5]{mccool2012structured}.

Lastly, we have also added an optimization where 
trees can be constructed in-place, reusing the existing nodes and structure
of the trees from the previous step. In order to employ this, the bounding box 
of all the points must be scaled up slightly so that the size of the root node
does not change at every step. Only when the root node changes size
do the trees need to be truly created from scratch again.
With the octree built and costzones computed, it is now
straightforward to compute the forces on each particle in parallel, 
using one thread per costzone.


\subsection{C++ Thread Support for Parallelism}
\label{sec:cppparallel}

For each step in the $N$-body simulation there are several
distinct parallel steps. There is the map-reduce
creation of the global octree, the force computation, and the integration step.
To spawn and join threads for each of these steps would lead
to too much overhead. %except in the case of extremely large values of $N$.
Instead, we employ a \textit{thread pool}---a collection of long-running
threads which wait to be given a task, execute that task, 
and then return to the pool. This avoids
the overhead of repeatedly spawning threads. 
Often, threads in a pool execute some statically-determined task.
However, our threads must be receptive to each of parallel steps.
We thus implement \textit{functor}-executing threads.
A functor is simply an object encoding a function call. 
Thus, these threads may execute any function that can be 
encapsulated as a functor.
To facilitate the object passing of functors to threads, 
we have implemented an asynchronous producer-consumer queue.
Nonetheless, these are all standard constructs in modern multithreaded programming, 
so we exclude further details.

Our threads, functors, and asynchronous queues are all built
using standard features of C++11. In particular, 
\texttt{std::thread} (which wraps \texttt{pthread} on Linux), 
\texttt{std:function} for functor objects, 
and \texttt{std::condition\_variable} for sleeping and 
waking threads waiting for a new functor.


\subsection{Three Dimensional Visualization}
\label{sec:ogl}

For both debugging and the natural beauty of it, 
we have implemented a visualization tool for 
our three-dimensional $N$-body simulation 
using OpenGL. This visualization tool
has already been shown in Figure~\ref{fig:ogltwoclusters}
where the collision of two star clusters is being simulated.
%%
The overall scene is rather simple. There is a camera whose
sight is fixed at the origin, but can rotate and zoom freely.
The origin is augmented with axes which act as a reference point
during movement. The x-y plane is given a translucent 
grid to give both scale to the simulation and a reference point
in the otherwise black space. The most interesting detail here 
is the implementation of the bodies in the space.

At each time-step in the simulation the positions of the bodies
are passed to the visualization tool for rendering.
Each is rendered as single point but using a number of shaders.
There are three rendering passes of importance.
The first renders a small two-dimensional Gaussian texture at each point.
This gives the appearance of \textit{limb-darkening}---where the 
central part of a star appears brighter than the edges.
The next pass slightly blurs each texture for a subtle haze and twinkle 
around each point. Finally, lighting bloom is calculated
where each point acts as a light source, creating the impression of 
ambient light in the inter-particle space.
Lastly, it may appear that the color of each body is random, 
but it is only to a point. In fact, we interpolate the apparent
color of main sequence stars from red through orange and white to blue.
In equal-mass simulations, a random color assignment in this interpolated range
gives visual interest and the ability to visually track a body over time.
Otherwise, one could assign color based on the mapping between mass and temperature.

